Is Precise Recovery Necessary? A Task-Oriented Imputation Approach for Time Series Forecasting on Variable Subset

Variable Subset Forecasting (VSF) refers to a unique scenario in multivariate time series forecasting, where available variables in the inference phase are only a subset of the variables in the training phase. VSF presents significant challenges as the entire time series may be missing, and neither inter- nor intra-variable correlations persist. Such conditions impede the effectiveness of traditional imputation methods, primarily focusing on filling in individual missing data points. Inspired by the principle of feature engineering that not all variables contribute positively to forecasting, we propose Task-Oriented Imputation for VSF (TOI-VSF), a novel framework shifts the focus from accurate data recovery to directly support the downstream forecasting task. TOI-VSF incorporates a self-supervised imputation module, agnostic to the forecasting model, designed to fill in missing variables while preserving the vital characteristics and temporal patterns of time series data. Additionally, we implement a joint learning strategy for imputation and forecasting, ensuring that the imputation process is directly aligned with and beneficial to the forecasting objective. Extensive experiments across four datasets demonstrate the superiority of TOI-VSF, outperforming baseline methods by $15\%$ on average.

==> table/table1-overall-4.tex <==
\begin{table*}[!t]
\small
\setlength\tabcolsep{6.6pt}
\caption{An illustration of the overall performance of time series forecasting on subset variables. 
The results are reported as an average and standard deviations (values in parenthesis) of 12 runs. 
Each run corresponds to one trained model with 100 epochs, and each epoch involves a randomly sampled variable subset.
% The values represent the average over 12 runs. (The numbers in parenthesis are corresponding standard deviations.) 
% The value represents the actual metrics over different settings. 
$\Delta_{subset}$ represents the improvement of our model over the partial setting. For the $\Delta_{subset}$, the larger the value, the better the performance.}
\begin{tabular}{c|c|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{\multirow{2.7}{*}{forecasting model}  }        & \multicolumn{2}{c|}{METR-LA}                 & \multicolumn{2}{c|}{Traffic}                 & \multicolumn{2}{c|}{SOLAR}                   & \multicolumn{2}{c}{ECG5000}                 \\

\cmidrule{3-10}
\multicolumn{2}{c|}{}                                       & MAE                  & RMSE                 & MAE                  & RMSE                 & MAE                  & RMSE                 & MAE                  & RMSE                 \\
\midrule
\multirow{5}{*}{ASTGCN}         & partial                   & 5.57(0.72)           & 10.61(1.36)          & 22.44(1.58)          & 43.07(2.46)          & 6.14(1.29)           & 8.95(2.35)           & 3.60(0.60)           & 6.05(1.13)           \\
& oracle                                         & 5.04(0.39)           & 9.59(0.62)           & 19.17(0.91)          & 40.21(2.02)          & 4.54(0.47)           & 6.48(0.85)           & 3.47(0.50)           & 5.83(0.99)           \\
& ours                                             & \textbf{4.09(0.28)}  & \textbf{8.24(0.59)}  & \textbf{17.11(1.04)} & \textbf{35.92(2.28)} & \textbf{3.37(0.42)}  & \textbf{5.11(0.68)}  & \textbf{3.13(0.46)}  & \textbf{5.47(1.08)}  \\

\cmidrule{2-10}
& {$\Delta_{subset}$}     & 26.50\%              & 22.34\%              & 23.76\%              & 16.60\%              & 45.19\%              & 42.86\%              & 13.01\%              & 9.59\%               \\
\midrule
\multirow{5}{*}{MSTGCN}         & partial                   & 4.78(0.43)           & 9.35(0.75)           & 18.96(1.21)          & 40.13(2.67)          & 4.75(0.73)           & 7.02(1.42)           & 4.43(0.87)           & 7.61(1.86)           \\
& oracle                                           & 4.49(0.31)           & 8.93(0.50)           & 17.41(0.74)          & 37.84(1.88)          & 3.64(0.41)           & 5.60(0.82)           & 3.39(0.52)           & 5.82(1.06)           \\
& ours                                             & \textbf{4.16(0.36)}  & \textbf{8.30(0.66)}  & \textbf{16.50(0.47)} & \textbf{34.39(1.08)} & \textbf{3.31(0.42)}  & \textbf{5.04(0.59)}  & \textbf{3.33(0.76)}  & \textbf{5.75(1.41)}  \\

\cmidrule{2-10}
& {$\Delta_{subset}$}     & 12.89\%              & 11.24\%              & 12.98\%              & 14.31\%              & 30.29\%              & 28.26\%              & 24.73\%              & 24.48\%              \\
\midrule
\multirow{5}{*}{MTGNN}          & partial                   & 4.54(0.37)           & 8.9(0.68)            & 18.57(2.31)          & 38.46(3.94)          & 4.36(0.53)           & 6.04(0.81)           & 3.88(0.61)           & 6.54(1.10)           \\
& oracle                                          & 3.49(0.25)           & 7.21(0.50)           & 11.45(0.57)          & 27.48(2.14)          & 2.94(0.27)           & 4.66(0.57)           & 3.43(0.54)           & 5.94(1.08)           \\
& ours                                             & \textbf{3.07(0.19)} & \textbf{6.36(0.36)}  & \textbf{11.32(0.54)} & \textbf{26.87(1.48)} & \textbf{2.74(0.21)} & \textbf{4.16(0.43)} & \textbf{3.35(0.47)} & \textbf{5.43(0.96)} \\

\cmidrule{2-10}
& {$\Delta_{subset}$}     & 32.38\%             & 28.54\%              & 39.03\%              & 30.13\%              & 37.15\%             & 31.15\%             & 13.75\%             & 16.98\%             \\
\midrule
\multirow{5}{*}{TGCN}           & partial                  & 8.04(0.62)          & 13.14(0.95)          & 38.58(2.07)          & 63.27(2.86)          & 6.45(1.07)          & 9.05(1.99)          & 6.76(1.69)          & 9.67(2.05)          \\
& oracle                                          & 7.73(0.94)          & 12.59(1.62)          & 26.35(1.32)          & 49.72(2.99)          & 5.43(0.23)          & 8.00(0.77)          & 5.60(1.82)          & 9.28(3.16)          \\
& ours                                             & \textbf{5.45(0.55)}  & \textbf{10.39(0.79)} & \textbf{20.37(1.20)} & \textbf{44.20(3.04)} & \textbf{4.51(0.75)}  & \textbf{7.26(1.54)}  & \textbf{4.81(0.95)}  & \textbf{8.04(2.01)}  \\

\cmidrule{2-10}
& {$\Delta_{subset}$}     & 32.35\%             & 20.92\%              & 47.20\%              & 30.15\%              & 30.00\%             & 19.78\%              & 28.82\%             & 16.85\%             \\
\midrule
\midrule
\multicolumn{2}{c|}{Average Improvement}                                             & \textbf{26.03\%}    & \textbf{20.76\%}     & \textbf{28.06\%}     & \textbf{22.80\%}     & \textbf{35.66\%}    & \textbf{30.51\%}    & \textbf{20.08\%}    & \textbf{16.98\%} \\

\bottomrule
\end{tabular}
\label{tab: overall performance}
% \vspace{-5mm}
\end{table*}

==> table/table2-oracle-4.tex <==
\begin{table*}[!h]

\centering
% \footnotesize
% \scriptsize
\small
\setlength\tabcolsep{10.6pt}
\caption{Relative performance to \textit{Oracle} setting. $\Delta_{improve}$ indicates the proportion by which our model surpasses the \textit{Oracle} setting. For the $\Delta_{improve}$, the larger the value, the better the performance.}
\begin{tabular}{c|c|cc|cc|cc|cc}
\toprule
\multicolumn{2}{c|}{\multirow{2.7}{*}{forecasting model}  }& \multicolumn{2}{c|}{METR-LA} & \multicolumn{2}{c|}{Traffic} & \multicolumn{2}{c|}{SOLAR} & \multicolumn{2}{c}{ECG5000} \\
\cmidrule{3-10}
\multicolumn{2}{c|}{}& MAE  & RMSE    & MAE  & RMSE  & MAE  & RMSE & MAE  & RMSE   \\
\midrule
ASTGCN  & $\Delta_{improve}$& 18.77\%      & 14.07\%      & 10.76\%                        & 10.67\%                       & 25.88\%     & 21.07\%     & 9.75\%       & 6.18\%       \\
\midrule
MSTGCN  & $\Delta_{improve}$& 7.27\%       & 7.06\%       & 5.24\%                         & 9.12\%                        & 9.03\%      & 10.07\%     & 1.64\%       & 1.26\%       \\
\midrule
MTGNN  & $\Delta_{improve}$& 12.03\%      & 11.79\%      & 1.11\% & 2.22\% & 6.79\%      & 10.76\%     & 2.43\%       & 8.59\%       \\
\midrule
TGCN  & $\Delta_{improve}$& 29.46\%      & 17.42\%      & 22.70\%                        & 11.11\%                       & 16.91\%     & 9.29\%      & 14.04\%      & 13.35\%      \\
\midrule
\midrule
% \multicolumn{2}{c|}{Average Improvement}& 16.88\% & 12.59\% & 9.95\%  & 8.28\% & 14.65\% & 12.80\%  & 6.97\% & 7.35\% \\
\multicolumn{2}{c|}{Average Improvement}& \multicolumn{1}{r}{\textbf{16.88\%}} & \multicolumn{1}{r}{\textbf{12.59\%}} & \multicolumn{1}{r}{\textbf{9.95\%}} & \multicolumn{1}{r}{\textbf{8.28\%}} & \multicolumn{1}{r}{\textbf{14.65\%}} & \multicolumn{1}{r}{\textbf{12.80\%}} & \multicolumn{1}{r}{\textbf{6.97\%}} & \multicolumn{1}{r}{\textbf{7.35\%}} \\
\bottomrule

\end{tabular}
% \vspace{-0.2cm}
% \caption{Relative performance to \textit{oracle} setting. $\Delta_{improve}$ indicates the proportion by which our model surpasses the \textit{oracle} setting.}
% \vspace{-9mm}
\label{tab:oracle-ours}
% \vspace{-2mm}
\end{table*}
